Identifying Surface Degeneracies in Single-Visit Reflected Light Observations of Modern Earth using the Habitable Worlds Observatory

Characterizing the surface and atmosphere of Earth-like planets in reflected light is a key goal for upcoming direct imaging surveys. NASA's next flagship-class astrophysics mission concept, the Habitable Worlds Observatory (HWO), is a space-based Ultraviolet/Optical/Near-Infrared observatory with a mission design requirement to reach the $10^{-10}$ contrast necessary to characterize Earth-like planets around Sun-like stars. While reflected light from planetary surfaces provides a unique opportunity to constrain the coverage of surface materials and biopigments, detailed predictions of HWO's ability to retrieve surface fractions are necessary but have not been conducted. Here, we model photon-counting noise from astrophysical, instrumental, and post-processing sources for the HWO Exploratory Analytic Case 5 design equipped with a charge-6 vector-vortex coronagraph. By combining our photon-counting noise with five distinct modern Earth models at quadrature, we simulate single-visit HWO observations and perform spectral retrievals using the open-source code $\texttt{POSEIDON}$ to assess our ability to constrain both the surface and atmospheric composition. We find that degeneracies between planetary radius, surface pressure, surface material, and cloud coverage in reflected-light retrievals can significantly complicate the classification of surface features. These degeneracies can complicate the detection of surface biopigments, such as the chlorophyll-induced red edge on modern Earth. Our work shows that developing concrete strategies for detecting surface features and breaking degeneracies in reflected-light observations of Earth-like planets is a critical priority for mission design and data analysis.

==> MODIS_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\caption{\label{tab:modis}Earth fractional coverage using IGPB classification scheme and the spectra used to represent each component. Spectra were primarily sourced from USGS \cite{kokaly_usgs_2017} and ECOSTRESS \cite{meerdink_ecostress_2019}, with the exception of snow\cite{grenfell_reflection_1994} and cropland\cite{jennewein_spaceborne_2024}. Multiple spectra types under the ``Spectral Representation'' column indicate an equal weighting of the spectra.}
%\begin{tabular}{@{}lccc@{}}
\noindent\begin{tabularx}{\linewidth}{@{}L{0.3\textwidth}ccC{0.11\textwidth}@{}}
\toprule
IGBP Classification                & Coverage (\%) & Spectral Representation                                                                           & Spectra Reference \\ \midrule
Water                              & 71.57         & Ocean                                                                                             &\citenum{kokaly_usgs_2017}\\
Evergreen Needleleaf Forest        & 0.49          & Englemann                                                                                         &\citenum{kokaly_usgs_2017}\\
Evergreen Broadleaf Forest         & 2.36          & Magnolia Grandiflora                                                                              &\citenum{meerdink_ecostress_2019}\\
Deciduous Needleleaf Forest        & 0.09          & Engelmann                                                                                         &\citenum{kokaly_usgs_2017}\\
Deciduous Broadleaf Forest         & 0.58          & Aspen                                                                                             &\citenum{kokaly_usgs_2017}\\
Mixed Forest                       & 0.93          & \begin{tabular}[c]{@{}c@{}}Engelmann, Aspen, \\ Magnolia Grandiflora\end{tabular}                 &\citenum{kokaly_usgs_2017, meerdink_ecostress_2019}\\
Closed Shrubland                   & 0.12          & \begin{tabular}[c]{@{}c@{}}Adenostoma fasciculatum,\\ Reddish brown fine sandly loam\end{tabular} &\citenum{meerdink_ecostress_2019}\\
Open Shrubland                     & 2.57          & \begin{tabular}[c]{@{}c@{}}Adenostoma fasciculatum,\\ Reddish brown fine sandly loam\end{tabular} &\citenum{meerdink_ecostress_2019}\\
Woody Savanna                      & 2.24          & Acacia Visco                                                                                      &\citenum{meerdink_ecostress_2019}\\
Savanna                            & 3.14          & Rangeland                                                                                         &\citenum{kokaly_usgs_2017}\\
Grassland                          & 5.99          & Rangeland                                                                                         &\citenum{kokaly_usgs_2017}\\
Permanent Wetland                  & 0.30          & Wetland                                                                                           &\citenum{kokaly_usgs_2017}\\
Cropland                           & 2.31          & Fresh Cut Wheat Residue                                                                           &\citenum{jennewein_spaceborne_2024}\\
Urban and Built-Up                 & 0.17          & Asphaltic Concrete                                                                                &\citenum{meerdink_ecostress_2019}\\
Cropland/Natural Vegetation Mosaic & 0.28          & Fresh Cut Wheat Residue                                                                           &\citenum{jennewein_spaceborne_2024}\\
Snow and Ice                       & 2.87          & Antarctic                                                                                         &\citenum{grenfell_reflection_1994}\\
Barren or Sparsely Vegetated       & 3.99          & Quartz Ottawa Sand                                                                                &\citenum{kokaly_usgs_2017}\\ \bottomrule
%\end{tabular}
\end{tabularx}
\end{table*}

==> atmo_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\caption{Summary of parameters used to model the three self-consistent {\tt POSEIDON} Earth-like exoplanet spectra and retrievals.}\label{tab:atmo}
\begin{tabular}{@{}lccc@{}}
\toprule
Variable                    & Unit & Input & Retrieval Prior \\  
\midrule Star & & & \\ \midrule
$T_{\rm eff}$   &   K   &   5772    & --- \\
$\logt g$ & cm/s$^2$    &   4.4 &   --- \\
${\rm[Fe/H]}$  &   dex &   0   &   --- \\
\midrule Planet & & & \\ \midrule
$R_p$                       & $R_{\oplus}$ & 1  & $\mathcal{U}(0.1,~10)$     \\
$\logt P_{\rm surf}$              & bar  & 0 & $\mathcal{U}(-3,~2)$  \\
$T$                         & K & 300 & $\mathcal{U}(100,~400)$ \\
$\alpha$    & degree  & 90 & --- \\
$r_p$ &   AU    & 1   &   ---\\
\midrule Mixing Ratios & & & \\ \midrule
$\logt{\rm H}_2{\rm O}$ &---& -3    & $\mathcal{U}(-12,~0)$ \\
$\logt{\rm O}_3$        &---& -6    & $\mathcal{U}(-12,~0)$\\
$\logt{\rm O}_2$        &---& -0.7    & $\mathcal{U}(-12,~0)$ \\
% \midrule PT Profile & & & \\ \midrule
% $T_{\rm high}$              & K    & 170   &$\mathcal{U}(200,~400)$ \\
% $T_{\rm mid}$               & K    & 200   & $\mathcal{U}(200,~400)$ \\
% $T_{\rm deep}$              & K    & 350   & $\mathcal{U}(200,~400)$ \\
% $\logt P_{\rm high}$         & bar  & -5    &    ---         \\
% $\logt P_{\rm mid}$          & bar  & -1    & $\mathcal{U}(-6,~1)$  \\
% $\logt P_{\rm deep}$         & bar  & 1     &  ---           \\
\midrule H$_2$O Clouds & & & \\ \midrule
$f_{\rm cloud}$  & --- & (0, 0.5, 1) & $\mathcal{U}(0,~1)$   \\
$\logt P_{\rm top}$  & bar & $\logt(0.5)$ & $\mathcal{U}(-4,~0)$   \\
$\Delta \logt P$  & bar & $\logt(1.2)$ & $\mathcal{U}(0.1,~3)$ \\
$\logt r_{m}$  & $\mu {\rm m}$ & $ 0$ & $\mathcal{U}(-1,~1)$ \\
$\logt {\rm H_2O}$  & --- & -3 & $\mathcal{U}(-8,~0)$ \\
\midrule Surface & & & \\ \midrule
$f_{\rm forest}$  & --- & 0.15 & $\mathcal{U}(0,~1)$   \\ 
$f_{\rm ocean}$   &---  & 0.7 &$\mathcal{U}(0,~1)$\\ 
$f_{\rm snow}$   &--- & 0.05 & $\mathcal{U}(0,~1)$  \\ 
$f_{\rm sand}$  & --- &  0.1 & $\mathcal{U}(0,~1)$  \\ 
\bottomrule
\end{tabular}
\end{table}

==> ref_header.tex <==
\newcommand\aj{{AJ}}%        % Astronomical Journal 
\newcommand\psj{{PSJ}}%       % Planetary Science Journal
\newcommand\araa{{ARA\&A}}%  % Annual Review of Astron and Astrophys 
\newcommand\apj{{ApJ}}%    % Astrophysical Journal 
\newcommand\apjl{{ApJL}}     % Astrophysical Journal, Letters 
\newcommand\apjs{{ApJS}}%    % Astrophysical Journal, Supplement 
\newcommand\ao{{ApOpt}}%   % Applied Optics 
\newcommand\apss{{Ap\&SS}}%  % Astrophysics and Space Science 
\newcommand\aap{{A\&A}}%     % Astronomy and Astrophysics 
\newcommand\aapr{{A\&A~Rv}}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{{A\&AS}}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{{AZh}}%       % Astronomicheskii Zhurnal 
\newcommand\baas{{BAAS}}%     % Bulletin of the AAS 
\newcommand\icarus{{Icarus}}% % Icarus
\newcommand\jaavso{{JAAVSO}}  % The Journal of the American Association of Variable Star Observers
\newcommand\jrasc{{JRASC}}%   % Journal of the RAS of Canada 
\newcommand\memras{{MmRAS}}%  % Memoirs of the RAS 
\newcommand\mnras{{MNRAS}}%   % Monthly Notices of the RAS 
\newcommand\pra{{PhRvA}}% % Physical Review A: General Physics 
\newcommand\prb{{PhRvB}}% % Physical Review B: Solid State 
\newcommand\prc{{PhRvC}}% % Physical Review C 
\newcommand\prd{{PhRvD}}% % Physical Review D 
\newcommand\pre{{PhRvE}}% % Physical Review E 
\newcommand\prl{{PhRvL}}% % Physical Review Letters 
\newcommand\pasp{{PASP}}%     % Publications of the ASP 
\newcommand\pasj{{PASJ}}%     % Publications of the ASJ 
\newcommand\qjras{{QJRAS}}%   % Quarterly Journal of the RAS 
\newcommand\skytel{{S\&T}}%   % Sky and Telescope 
\newcommand\solphys{{SoPh}}% % Solar Physics 
\newcommand\sovast{{Soviet~Ast.}}% % Soviet Astronomy 
\newcommand\ssr{{SSRv}}% % Space Science Reviews 
\newcommand\zap{{ZA}}%       % Zeitschrift fuer Astrophysik 
\newcommand\nat{{Nature}}%  % Nature 
\newcommand\iaucirc{{IAUC}}% % IAU Cirulars 
\newcommand\aplett{{Astrophys.~Lett.}}%  % Astrophysics Letters 
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}% % Astrophysics Space Physics Research 
\newcommand\bain{{BAN}}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{{FCPh}}%   % Fundamental Cosmic Physics 
\newcommand\gca{{GeoCoA}}% % Geochimica Cosmochimica Acta 
\newcommand\grl{{Geophys.~Res.~Lett.}}%  % Geophysics Research Letters 
\newcommand\jcp{{JChPh}}%     % Journal of Chemical Physics 
\newcommand\jgr{{J.~Geophys.~Res.}}%     % Journal of Geophysics Research 
\newcommand\jqsrt{{JQSRT}}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\nphysa{{NuPhA}}%     % Nuclear Physics A 
\newcommand\physrep{{PhR}}%       % Physics Reports 
\newcommand\physscr{{PhyS}}%        % Physica Scripta 
\newcommand\planss{{Planet.~Space~Sci.}}%  % Planetary Space Science 
\newcommand\procspie{{Proc.~SPIE}}%      % Proceedings of the SPIE 

\newcommand\actaa{{AcA}}%  % Acta Astronomica
\newcommand\caa{{ChA\&A}}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{{ChJA\&A}}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{{JCAP}}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{{NewA}}%  % New Astronomy
\newcommand\nar{{NewAR}}%  % New Astronomy Review
\newcommand\pasa{{PASA}}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{{RMxAA}}%  % Revista Mexicana de Astronomia y Astrofisica

%% added feb 9, 2016
\newcommand\maps{{M\&PS}}% Meteoritics and Planetary Science
\newcommand\aas{{AAS Meeting Abstracts}}% American Astronomical Society Meeting Abstracts
\newcommand\dps{{AAS/DPS Meeting Abstracts}}% American Astronomical Society/Division for Planetary Sciences Meeting Abstracts



\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

==> surface_spec_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\caption{Surface spectra used in this study, as well as their percent surface coverage in the MODIS-derived surface spectra.}\label{tab:surf}
% \begin{tabular}{@{}lccll@{}}
\noindent\begin{tabularx}{\linewidth}{@{}L{0.17\linewidth}ccL{0.31\linewidth}l@{}}
\toprule
Surface Name                   & Coverage (\%) & Reference                           & Source Spectrum Name/Location            & ID          \\ \midrule
Ocean                          & 71.57            & \citenum{kokaly_usgs_2017}          & Seawater\_Open\_Ocean SW2 lwch BECKa AREF  & SW1         \\
Aspen                          & 0.89             & \citenum{kokaly_usgs_2017}          & Aspen Aspen-1 green-top ASDFRa AREF      & Aspen-1     \\
Engelmann                      & 0.89             & \citenum{kokaly_usgs_2017}          & Engelmann-Spruce ES-Needls-1 ASDFRa AREF & ES-Needls-1 \\
Magnolia Grandiflora           & 2.67             & \citenum{meerdink_ecostress_2019}   & Magnolia grandiflora                     & JPL231      \\
Adenostoma Fasciculatum        & 0.81             & \citenum{meerdink_ecostress_2019}   & Adenostoma fasciculatum 1                & VH217       \\
Reddish brown fine sandy loam & 1.89             & \citenum{meerdink_ecostress_2019}   & Reddish brown fine sandy loam            & 87P1087     \\
Acacia Visco                   & 2.24             & \citenum{meerdink_ecostress_2019}   & Acacia visco                             & JPL159      \\
Rangeland                      & 9.13             & \citenum{kokaly_usgs_2017}          & Rangeland L02-069 S00\% G99\% ASDFRa AREF  & L02-069     \\
Wetland                        & 0.3              & \citenum{kokaly_usgs_2017}          & Wetland YNP-WT-1 AVIRISb RTGC            & YNP-WT-1    \\
Wheat Residue                  & 2.59             & \citenum{jennewein_spaceborne_2024} & Wheat, Field Scale Cut Green             & 33          \\
Asphalt                        & 0.17             & \citenum{meerdink_ecostress_2019}   & Construction Asphalt                     & 0674UUUASP  \\
Antarctic                      & 2.87             & \citenum{grenfell_reflection_1994}  & Table. 6                                 & ---         \\
Sand                           & 3.99             & \citenum{kokaly_usgs_2017}          & Quartz GDS74 Sand Ottawa BECKc AREF      & GDS74 Sand  \\ \bottomrule
% \end{tabular}
\end{tabularx}
\end{table*}

==> tele_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{\label{tab:tele}
Parameters assumed for modeling the HWO EAC 5 design. Values are adopted from the GOMAP Science-Engineering Interface repository if available and filled with values from the LUVOIR report\cite{the_luvoir_team_luvoir_2019}.}
\begin{tabular}{@{}lllll@{}}
\toprule
Parameter                                      & Description                 & Unit                    & \multicolumn{1}{l}{VIS} & \multicolumn{1}{l}{NIR} \\ \midrule
$D_{\rm circ}$                                              & Circumscribed diameter          & m                       & \multicolumn{2}{c}{10}           \\
$D_{\rm in}$                                              & Inscribed diameter          & m                       & \multicolumn{2}{c}{8.3}    \\
$A$                                              & Collecting area          & ${\rm m}^2$                       & \multicolumn{2}{c}{65.4}    \\
$C$                                              & Coronagraph design contrast &  ---   & \multicolumn{2}{c}{$10^{-10}$}                    \\
$\mathcal{R}$                                  & Spectral resolution                  & --- & 140                     & 70              \\
$[\lambda_\mathrm{min}, \lambda_\mathrm{max}]$ & Wavelength range            & $\mu{\rm m}$            & {[}0.4,1.0{]}           & {[}1.0,1.8{]}           \\
$\theta_{\rm OWA}$                             & Outer working angle         & $\lambda/D$             & \multicolumn{2}{c}{32}                            \\
$\theta_{\rm IWA}$                             & Inner working angle         & $\lambda/D$             & \multicolumn{2}{c}{2.5}                           \\
$f_{\rm pp}$                             & Post-processing factor         & ---             & \multicolumn{2}{c}{0.1}                           \\
$T_{\mathrm{sys}}$                             & Telescope temperature       & K                       & \multicolumn{2}{c}{270}                           \\
$t_{\rm exp}$                                  & Exposure time               & hr                    & \multicolumn{2}{c}{100}                           \\
$t_{\rm read}$                                  & Read time               & s                    & \multicolumn{2}{c}{1000}                           \\
$R_\mathrm{e^-}$                               & Read noise                  & $\mathrm{ e^-}$/pixel   & 0                       & 0.4                     \\
$D_\mathrm{e^-}$                               & Dark current                & $\mathrm{ e^-}$/pixel/s & $3\times 10^{-5}$       & $1\times 10^{-4}$       \\
$R_\mathrm{C}$                                 & Clock induced charge        & $\mathrm{ e^-/pixel}$   & \multicolumn{2}{c}{$1.3\times 10^{-3}$}           \\ \bottomrule
\end{tabular}
\end{table}
